A Coinductive Version of Milner's Proof System for Regular Expressions Modulo Bisimilarity

By adapting Salomaa's complete proof system for equality of regular expressions under the language semantics, Milner (1984) formulated a sound proof system for bisimilarity of regular expressions under the process interpretation he introduced. He asked whether this system is complete. Proof-theoretic arguments attempting to show completeness of this equational system are complicated by the presence of a non-algebraic rule for solving fixed-point equations by using star iteration. We characterize the derivational power that the fixed-point rule adds to the purely equational part $\text{Mil$^{\boldsymbol{-}}$}$ of Milner's system $\text{$\text{Mil}$}$: it corresponds to the power of coinductive proofs over $\text{Mil$^{\boldsymbol{-}}$}$ that have the form of finite process graphs with the loop existence and elimination property $\text{LEE}$. We define a variant system $\text{cMil}$ by replacing the fixed-point rule in $\text{Mil}$ with a rule that permits $\text{LEE}$-shaped circular derivations in $\text{Mil$^{\boldsymbol{-}}$}$ from previously derived equations as a premise. With this rule alone we also define the variant system $\text{CLC}$ for merely combining $\text{LEE}$-shaped coinductive proofs over $\text{Mil$^{\boldsymbol{-}}$}$. We show that both $\text{cMil}$ and $\text{CLC}$ have proof interpretations in $\text{Mil}$, and vice versa. As this correspondence links, in both directions, derivability in $\text{Mil}$ with derivation trees of process graphs, it widens the space for graph-based approaches to finding a completeness proof of Milner's system. This report is the extended version of a paper with the same title presented at CALCO 2021.

==> figs/.jle/history/fig-ex-extraction-proof.tex <==
\begin{figure}[tbp]
  %
\begin{center}
  $
  \hspace*{-3ex}%
  \begin{aligned}
    \scalebox{0.9}{\input{figs/fig-ex-coindproof-short.tex}}
  \end{aligned}
  %
  \hspace*{1ex}
  %
  \begin{aligned}[c]
    \aeqfuni{i}{\averti{21}}
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\eqinsol{\milnersysmin}$}\,
    \stexpprod{\stexpone}{\aeqfuni{i}{\averti{2}}} 
      \,\milnersysmineq\,
    \aeqfuni{i}{\averti{2}} 
    \\[-0.75ex]
      & \phantom{\;\parbox[t]{\widthof{$\milnersysmineq$}}{$\eqinsol{\milnersysmin}$}}\,
        \text{($\eqinsol{\milnersysmin}$ means use of 
               `is \provablein{\milnersysmin} solution')}
    \\
    \aeqfuni{i}{\averti{2}}
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\eqinsol{\milnersysmin}$}\,
    \stexpsum{\stexpprod{\bact}{\aeqfuni{i}{\averti{21}}}}
             {\stexpprod{\stexpone}{\aeqfuni{i}{\start}}} 
      \,\milnersysmineq\,
    \stexpsum{\stexpprod{\bact}{\aeqfuni{i}{\averti{2}}}}
             {\aeqfuni{i}{\start}}
    \\[-0.5ex]
    & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\Downarrow${\text{~~applying $\RSPstar$}}}
    \\[-0.5ex]
    \aeqfuni{i}{\averti{2}}
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersyseq$}\,
    \stexpprod{\stexpit{\bact}}
              {\aeqfuni{i}{\start}}
    %
    \\[0.5ex]
    %
    \aeqfuni{i}{\averti{11}}
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\eqinsol{\milnersysmin}$}\,
    \stexpprod{\stexpone}{\aeqfuni{i}{\averti{1}}} 
      \,\milnersysmineq\,
    \aeqfuni{i}{\averti{1}} 
    \\
    \aeqfuni{i}{\averti{1}}
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersysmineq$}\,
    \stexpsum{\stexpprod{\aact}{\aeqfuni{i}{\averti{11}}}}
             {\stexpsum{\stexpprod{\bact}{\aeqfuni{i}{\averti{21}}}}
                       {\stexpprod{\stexpone}{\aeqfuni{i}{\start}}}}
    % \\[-0.25ex]
    %   & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersysmineq$}\,
    % \stexpsum{\stexpprod{\aact}{\aeqfuni{i}{\averti{11}}}}
    %          {\stexpsum{\stexpprod{\bact}{\aeqfuni{i}{\averti{2}}}}
    %                    {\aeqfuni{i}{\start}}}
    \\[-0.25ex]      
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersyseq$}\,
    \stexpsum{\stexpprod{\aact}{\aeqfuni{i}{\averti{1}}}}
             {\stexpprod{(\stexpsum{\stexpprod{\bact}{\stexpit{\bact}}}
                                   {\stexpone})}
                        {\aeqfuni{i}{\start}}}
    \\[-0.25ex]      
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersysmineq$}\,
    \stexpsum{\stexpprod{\aact}{\aeqfuni{i}{\averti{1}}}}
             {\stexpprod{\stexpit{\bact}}
                        {\aeqfuni{i}{\start}}}
    \\[-0.5ex]
    & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\Downarrow${\text{~~applying $\RSPstar$}}}
    \\[-0.5ex]
    \aeqfuni{i}{\averti{1}}
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersyseq$}\,
    \stexpprod{\stexpit{\aact}}
              {(\stexpprod{\stexpit{\bact}}{\aeqfuni{i}{\start}})}
      \,\milnersysmineq\,          
    \stexpprod{(\stexpprod{\stexpit{\aact}}{\stexpit{\bact}})}{\aeqfuni{i}{\start}}  
    % %
    % \\[0.5ex]
    % %
    % \aeqfuni{i}{\start}
    %   & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\eqinsol{\milnersysmin}$}\,
    % 1 +  
    % \stexpsum{\stexpprod{\aact}{\aeqfuni{i}{\averti{11}}}}
    %          {\stexpprod{\bact}{\aeqfuni{i}{\averti{21}}}} 
    %   \,\milnersysmineq\,
    % 1 +  
    % \stexpsum{\stexpprod{\aact}{\aeqfuni{i}{\averti{1}}}}
    %          {\stexpprod{\bact}{\aeqfuni{i}{\averti{2}}}}   
    % \\[-0.25ex]
    %   & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersyseq$}\,
    % \stexpprod{(\stexpsum{\stexpprod{\aact}{(\stexpprod{\stexpit{\aact}}{\stexpit{\bact}})}}
    %                      {\stexpprod{\bact}{\stexpit{\bact}}})}
    %           {\aeqfuni{i}{\start}}
    %   + 1          
    % \\[-0.5ex]
    % & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\Downarrow${\text{~~applying $\RSPstar$}}}
    % \\[-0.5ex]
    % \aeqfuni{i}{\start}
    %   & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersyseq$}\,
    % \stexpprod{(\stexpsum{\stexpprod{\aact}{(\stexpprod{\stexpit{\aact}}{\stexpit{\bact}})}}
    %                      {\stexpprod{\bact}{\stexpit{\bact}}})}
    %           {\stexpone}
    %   \,\synteq\,
    % \extrsolof{\aonecharthat}{\start}            
  \end{aligned}
  $
  \\[0.75ex]
  $
  \begin{aligned}
    %
    \aeqfuni{i}{\start}
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\eqinsol{\milnersysmin}$}\,
    1 +  
    \stexpsum{\stexpprod{\aact}{\aeqfuni{i}{\averti{11}}}}
             {\stexpprod{\bact}{\aeqfuni{i}{\averti{21}}}} 
      \,\milnersysmineq\,
    1 +  
    \stexpsum{\stexpprod{\aact}{\aeqfuni{i}{\averti{1}}}}
             {\stexpprod{\bact}{\aeqfuni{i}{\averti{2}}}}   
    \\[-0.25ex]
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersyseq$}\,
    \stexpprod{(\stexpsum{\stexpprod{\aact}{(\stexpprod{\stexpit{\aact}}{\stexpit{\bact}})}}
                         {\stexpprod{\bact}{\stexpit{\bact}}})}
              {\aeqfuni{i}{\start}}
      + 1          
    \\[-0.5ex]
    & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\Downarrow${\text{~~applying $\RSPstar$}}}
    \\[-0.5ex]
    \aeqfuni{i}{\start}
      & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersyseq$}\,
    \stexpprod{\stexpit{(\stexpsum{\stexpprod{\aact}{(\stexpprod{\stexpit{\aact}}{\stexpit{\bact}})}}
                                  {\stexpprod{\bact}{\stexpit{\bact}}})}}
              {\stexpone}
      \,\milnersysmineq\,
    \stexpit{(\stexpsum{\stexpprod{\aact}{(\stexpprod{\stexpit{\aact}}{\stexpit{\bact}})}}
                       {\stexpprod{\bact}{\stexpit{\bact}}})}        
      \,\milnersysmineq\,
    \extrsolof{\aonecharthat}{\start}
  \end{aligned}
  $     
\end{center}
    \vspace*{-3ex}
\caption{\protect\label{fig:ex:extraction:proof}%
         Use of the \protect\LLEEwitness~$\protect\aonecharthat$ underlying the coinductive proof $\protect\pair{\protect\aonechart}{\protect\saeqfun}$ in Ex.~\protect\ref{ex:2:LLEEcoindproof}
         for showing that 
         the principal value $\protect\aeqfuni{i}{\protect\start}$ of the \protect\provablein{\protect\milnersysmin} solution $\protect\saeqfuni{i}$ for $i\protect\in\protect\setexp{1,2}$ 
         is \protect\provablyin{\protect\milnersys} is \protect\provablyin{\protect\milnersys} equal to the principal value $\protect\extrsolof{\protect\aonecharthat}{\protect\start}$ of the solution $\protect\sextrsolof{\protect\aonecharthat}$ 
         extracted from $\protect\aonecharthat$ (see Fig.~\protect\ref{fig:ex:extraction}). 
         }
  %
\end{figure}      

==> figs/.jle/history/fig-ex-extraction.tex <==
\begin{figure}[tbp]
  %
\begin{center}
  %
  \begin{equation*}
    %
    \hspace*{-3ex}
    \begin{aligned}[c]
      \scalebox{1.3}{\input{figs/fig-LLEEw-ex-extraction.tex}}
    \end{aligned}
    %
    \hspace*{1ex}
    %
    \begin{aligned}[c]
      \extrsoluntilof{\aonecharthat}{\averti{21}}{\averti{2}}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{\stexpzero}}  
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\averti{2}}{\averti{2}}})}
        \,\synteq\,
      \stexpprod{\stexpit{\stexpzero}}{(\stexpprod{\stexpone}{\stexpone})}
        \,\milnersysmineq\,
      \stexpone
      \\[-0.1ex]
      \extrsoluntilof{\aonecharthat}{\averti{2}}{\start}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{(\stexpprod{\bact}{\extrsoluntilof{\aonecharthat}{\averti{21}}{\averti{2}}})}}
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\start}{\start}})}
        \,\milnersysmineq\,  
      \stexpit{\bact}
      \\[-0.1ex]
      \extrsoluntilof{\aonecharthat}{\averti{21}}{\start}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{\stexpzero}}  
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\averti{2}}{\start}})}
        \,\milnersysmineq\,
      \stexpprod{\stexpone}{\stexpit{\bact}}
        \,\milnersysmineq\,
      \stexpit{\bact}
      %
      \\[-0.1ex]
      %
      \extrsoluntilof{\aonecharthat}{\averti{11}}{\averti{1}}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{\stexpzero}}
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\averti{1}}{\averti{1}}})}
        \,\synteq\,
      \stexpprod{\stexpit{\stexpzero}}
                {(\stexpprod{\stexpone}{\stexpone})}
        \,\milnersysmineq\,
      \stexpone
      \\[-0.1ex]
      \extrsoluntilof{\aonecharthat}{\averti{1}}{\start}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{(\stexpprod{\aact}{\extrsoluntilof{\aonecharthat}{\averti{11}}{\start}})}}
                {(\stexpsum{\stexpprod{\bact}{\extrsoluntilof{\aonecharthat}{\averti{21}}{\start}}}
                           {\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\start}{\start}}})}
      \\[-0.5ex] 
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersysmineq$}\,
      \stexpprod{\stexpit{\aact}}
                {(\stexpsum{\stexpprod{\bact}{\stexpit{\bact}}}
                           {\stexpone})}
        \,\milnersysmineq\,
      \stexpprod{\stexpit{\aact}}{\stexpit{\bact}} 
      \\[-0.1ex]
      \extrsoluntilof{\aonecharthat}{\averti{11}}{\start}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{\stexpzero}}  
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\averti{1}}{\start}})}
        \,\milnersysmineq\,
      % \stexpprod{\stexpit{\stexpzero}}{(\stexpprod{\stexpone}{\stexpprod{(\stexpit{\aact}}{\stexpit{\bact})}})}
      %  \,\milnersysmineq\,
      \stexpprod{\stexpit{\aact}}{\stexpit{\bact}}
      %
      \\[-0.1ex]
      \extrsolof{\aonecharthat}{\start}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{(\stexpsum{\stexpprod{\aact}{\extrsoluntilof{\aonecharthat}{\averti{11}}{\start}}}
                                    {\stexpprod{\bact}{\extrsoluntilof{\aonecharthat}{\averti{21}}{\start}}})}}
                {\stexpone}
      \\[-0.5ex]
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersysmineq$}\,
     \stexpit{(\stexpsum{\stexpprod{\aact}{(\stexpprod{\stexpit{\aact}}{\stexpit{\bact}})}}
                        {\stexpprod{\bact}{\stexpit{\bact}}})}
    \end{aligned}
    %
  \end{equation*}     
  %      
\end{center}
    \vspace*{-2.5ex}
  \caption{\protect\label{fig:ex:extraction}%
           Extraction of the principal value $\protect\extrsolof{\protect\aonecharthat}{\protect\start}$ of a \protect\provablein{\protect\milnersysmin} solution~$\protect\sextrsolof{\protect\aonecharthat}$ 
           from\protect\vspace*{-2pt} the \protect\LLEEwitness~$\protect\acharthat$ used for the coinductive proof 
           in Ex.~\protect\ref{ex:2:LLEEcoindproof}.
           We shorten solution values by using axioms~of~\protect\milnersysmin.
           }

  %
\end{figure}      

==> figs/fig-ex-coindproof-2-milnersys.tex <==
\begin{figure}[tbp]
  %
\begin{center}
  %
  \begin{equation*}
    %
    \hspace*{-3ex}
    \begin{aligned}[c]
      \scalebox{1.3}{\input{figs/fig-ex-coindproof-short.tex}}
    \end{aligned}
    %
    \hspace*{1ex}
    %
    \begin{aligned}[c]
      \extrsoluntilof{\aonecharthat}{\averti{21}}{\averti{2}}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{\stexpzero}}  
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\averti{2}}{\averti{2}}})}
        \,\synteq\,
      \stexpprod{\stexpit{\stexpzero}}{(\stexpprod{\stexpone}{\stexpone})}
        \,\milnersysmineq\,
      \stexpone
      \\
      \extrsoluntilof{\aonecharthat}{\averti{2}}{\avert}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{(\stexpprod{\bact}{\extrsoluntilof{\aonecharthat}{\averti{21}}{\averti{2}}})}}
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\avert}{\avert}})}
        \,\milnersysmineq\,  
      \stexpit{\bact}
      \\
      \extrsoluntilof{\aonecharthat}{\averti{21}}{\avert}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{\stexpzero}}  
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\averti{2}}{\avert}})}
        \,\milnersysmineq\,
      \stexpprod{\stexpone}{\stexpit{\bact}}
        \,\milnersysmineq\,
      \stexpit{\bact}
      %
      \\
      %
      \extrsoluntilof{\aonecharthat}{\averti{11}}{\averti{1}}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{\stexpzero}}
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\averti{1}}{\averti{1}}})}
        \,\synteq\,
      \stexpprod{\stexpit{\stexpzero}}
                {(\stexpprod{\stexpone}{\stexpone})}
        \,\milnersysmineq\,
      \stexpone
      \\
      \extrsoluntilof{\aonecharthat}{\averti{1}}{\avert}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{(\stexpprod{\aact}{\extrsoluntilof{\aonecharthat}{\averti{11}}{\avert}})}}
                {(\stexpsum{\stexpprod{\bact}{\extrsoluntilof{\aonecharthat}{\averti{21}}{\avert}}}
                           {\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\avert}{\avert}}})}
      \\[-0.5ex] 
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersysmineq$}\,
      \stexpprod{\stexpit{\aact}}
                {(\stexpsum{\stexpprod{\bact}{\stexpit{\bact}}}
                           {\stexpone})}
        \,\milnersysmineq\,
      \stexpprod{\stexpit{\aact}}{\stexpit{\bact}} 
      \\
      \extrsoluntilof{\aonecharthat}{\averti{11}}{\avert}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{\stexpzero}}  
                {(\stexpprod{\stexpone}{\extrsoluntilof{\aonecharthat}{\averti{1}}{\avert}})}
        \,\milnersysmineq\,
      % \stexpprod{\stexpit{\stexpzero}}{(\stexpprod{\stexpone}{\stexpprod{(\stexpit{\aact}}{\stexpit{\bact})}})}
      %  \,\milnersysmineq\,
      \stexpprod{\stexpit{\aact}}{\stexpit{\bact}}
      %
      \\
      \extrsolof{\aonecharthat}{\avert}
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\defdby$}\,
      \stexpprod{\stexpit{(\stexpsum{\stexpprod{\aact}{\extrsoluntilof{\aonecharthat}{\averti{11}}{\avert}}}
                                    {\stexpprod{\bact}{\extrsoluntilof{\aonecharthat}{\averti{21}}{\avert}}})}}
                {\stexpzero}
      \\[-0.5ex]
        & \;\parbox[t]{\widthof{$\milnersysmineq$}}{$\milnersysmineq$}\,
      \stexpprod{\stexpit{(\stexpsum{\stexpprod{\aact}{(\stexpprod{\stexpit{\aact}}{\stexpit{\bact}})}}
                                    {\stexpprod{\bact}{\stexpit{\bact}}})}}
                {\stexpzero}
    \end{aligned}
    %
  \end{equation*}     
  %      
\end{center}
    \vspace*{-1.5ex}
  \caption{\label{fig:ex:extraction}%
           Extraction of the principal value $\extrsolof{\aonecharthat}{\avert}$ of a \protect\provablein{\protect\milnersysmin} solution~$\sextrsolof{\aonecharthat}$ 
           from\vspace*{-2pt} the \protect\LLEEwitness~$\acharthat$ used for the coinductive proof 
           in Ex.~\ref{ex:2:LLEEcoindproof}.
           We shorten solution values by using axioms~of~\protect\milnersysmin.
           }

  %
\end{figure}      
